On the solvability of of some partial differential inequality

The \pn{Dulac} criterion is a classical method to rule out the existence of periodic solutions in planar differential equations. In this paper the applicability and therefore reversibility of this criterion is under consideration.

==> header.tex <==
% zur Kontrolle des Umbruchs Klassenoption draft verwenden

%\usepackage[ngerman]{babel}
%\usepackage[latin1]{inputenc}
%\input{psfig}
%\usepackage{ps4pdf}

% Seitenlayout
% DIV# gibt den Divisor für die Layoutberechnung an.
% Vergrößern des Divisors vergrößert den Textbereich.
% BCOR#cm gibt d Breite des Bundstegs an.
%\usepackage[DIV14,BCOR2cm]{typearea}

% Abstand obere Blattkante zur Kopfzeile ist 2.54cm - 15mm
\setlength{\topmargin}{-15mm}

% Umgebungen für Definitionen, Sätze, usw.
%\theoremstyle{plain}
\iffalse
\fi


\iffalse

\newcommand{\setC}{\mathbb{C}}
\newcommand{\setCm}{\mathbb{C^{-}}}

\newcommand{\setQ}{\mathbb{Q}}

\newcommand{\setT}{\mathbb{T}}
\newcommand{\setZ}{\mathbb{Z}}
\newcommand{\Range}{\matcal{R}}
\newcommand{\setL}{\mathcal{L}}
\newcommand{\setM}{\mathcal{M}}
\newcommand{\setB}{\mathcal{B}}
\newcommand{\setF}{\mathcal{F}}

\newcommand{\setO}{\mathcal{O}}
\newcommand{\setP}{\mathcal{P}}
\newcommand{\test}{\cont^{\infty}_{0}(\Omega)}

\newcommand{\om}{\omega}
\newcommand{\ve}{\varepsilon}
\newcommand{\vp}{\varphi}
\newcommand{\vr}{\varrho}
\newcommand{\vt}{\vartheta}
\newcommand{\Alpha}{\mathrm{A}}
\newcommand{\Beta}{\mathrm{B}}
\fi


\newcommand {\contLin}{\mathcal{L}}

%\newcommand \functions[2]{Abb_{#1,#2}}
%\newcommand \function[1]{Abb_{#1}}
\newcommand \term[1]{\textbf{#1}}
\newcommand \frage[1]{\textbf{Frage: }\emph{#1} }
\newcommand \beachte[1]{\textbf{beachte: }\emph{#1} }
\newcommand \gen[1]{\textbf{Generalvoraussetzung: }\emph{#1} }
%\newcommand \problem[3]{\textbf{#1}\textit{#2}\emph{#3}}

%\renewcommand{\glossaryname}{Syembolverzeichnis}

\DeclareMathOperator{\ind}{ind}
\DeclareMathOperator{\codim}{condim}

